Quasielastic $\overrightarrow{^{3}\mathrm{He}}(\overrightarrow{e},{e'})$ Asymmetry in the Threshold Region

A measurement of the double-spin asymmetry from electron-$^{3}$He scattering in the threshold region of two- and three-body breakup of $^{3}$He was performed at Jefferson Lab, for Q$^{2}$ values of 0.1 and 0.2 (GeV/$c$)$^{2}$. The results of this measurement serve as a stringent test of our understanding of few-body systems. When compared with calculations from plane wave impulse approximation and Faddeev theory, we found that the Faddeev calculations, which use modern nuclear potentials and prescriptions for meson-exchange currents, demonstrate an overall good agreement with data.

==> Makefile <==
DocName=Quasielastic
REV=NONE

TEXEXE=pdflatex -halt-on-error -file-line-error
#TEXEXE=xelatex

SHELL=/bin/bash

pdf: *.tex
	$(TEXEXE) $(DocName).tex
	bibtex $(DocName)
#	biber --quiet --output-safechars   $(DocName)
	$(TEXEXE) $(DocName).tex
	$(TEXEXE) $(DocName).tex

	@echo -e '\n\n                 ---------- WARNINGS ----------\n\n'
	grep Warning $(DocName).log | grep -v 'float specifier changed'
	@echo -e '\n\n                 ------------------------------\n\n'

diff:
ifeq ($(REV),NONE)
	@echo ''
	@echo 'Usage:  make REV=<git sha1>'
	@echo '    Use 'git log' and choose the commit you want to compare to.'
	@echo '    A new PDF will be generated with removals/addtions in red/blue.'
	@echo ''
else
	latexdiff-git --force --flatten --pdf -r $(REV) $(DocName).tex
endif

clean:
	rm -f $(DocName).{out,log,spl,bbl,blg,brf,lot,lof,toc} *.aux ${DocName}Notes.bib

realclean: clean
	rm -f $(DocName).pdf

#########################################################
# .gitignore for latex builds
#########################################################
# ## Ignore editor debris
# *~
# *.swp
# *.swo
# .#*
# [#]*[#]
# 
# ## Apple debris
# .DS_Store
# .AppleDouble
# .LSOverride
# 
# ## NFS temp files
# .nfs*
# 
# ## Auto generated files
# *.out
# *.aux
# *.bbl
# *.blg
# *.log
# *.spl
# *.lof
# *.lot
# *.toc
# *.glo
# *.ist
# thesis.pdf
# #########################################################


==> authorlist_2.tex <==
\author{M. Nycz$^{1*}$}
\email{mnycz@jlab.org}
\affiliation{University of Virginia, Charlottesville, Virginia 22904, USA} %make sure same institutions are using identical lines

\author{S. Barcus}
\affiliation{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, USA}

\author{M.~Cardona}
\affiliation{Temple University, Philadelphia, Pennsylvania 19122, USA}

\author{J.P.~Chen}
\affiliation{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, USA}

\author{J.~Chen}
\affiliation{College of William and Mary, Williamsburg, Virginia 23187, USA}

\author{M.~Chen}
\affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}

\author{A.~Deltuva}
\affiliation{Institute of Theoretical Physics and Astronomy, Vilnius University, Saule ̇tekio al. 3, LT-10257 Vilnius, Lithuania}

\author{J.~Golak}
\affiliation{Faculty of Physics, Astronomy and Applied Computer Science,
Jagiellonian University, PL-30348 Krak\'ow, Poland}

\author{D.W.~Higinbotham}
\affiliation{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, USA}

\author{W.~Korsch}
\affiliation{University of Kentucky, Lexington, Kentucky 40506, USA}

\author{S.~Li}
\affiliation{University of New Hampshire, Durham, New Hampshire 03824, USA}

\author{M.~Roy}
\affiliation{University of Kentucky, Lexington, Kentucky 40506, USA}

\author{P.U.~Sauer}
\affiliation{Institut f\"ur Theoretische Physik,  Universit\"at Hannover,D-30167 Hannover, Germany}

\author{S.~Scopeta}
\affiliation{Dipartimento di Fisica e Geologia, Università degli Studi di Perugia and Istituto Nazionale di Fisica Nucleare, Sezione di Perugia, via A. Pascoli, I - 06123 Perugia, Italy}

\author{R.~Skibi\'nski}
\affiliation{Faculty of Physics, Astronomy and Applied Computer Science,
Jagiellonian University, PL-30348 Krak\'ow, Poland}

\author{H.~Witała}
\affiliation{Faculty of Physics, Astronomy and Applied Computer Science,
Jagiellonian University, PL-30348 Krak\'ow, Poland}
\author{B.~Sawatzky}
\affiliation{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, USA}

\author{J.~Zhang}
\affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}

\author{X.~Zheng}%
\affiliation{University of Virginia, Charlottesville, Virginia 22904, USA}


